Massively Scaling Heteroscedastic Classifiers

Heteroscedastic classifiers, which learn a multivariate Gaussian distribution over prediction logits, have been shown to perform well on image classification problems with hundreds to thousands of classes. However, compared to standard classifiers, they introduce extra parameters that scale linearly with the number of classes. This makes them infeasible to apply to larger-scale problems. In addition heteroscedastic classifiers introduce a critical temperature hyperparameter which must be tuned. We propose HET-XL, a heteroscedastic classifier whose parameter count when compared to a standard classifier scales independently of the number of classes. In our large-scale settings, we show that we can remove the need to tune the temperature hyperparameter, by directly learning it on the training data. On large image classification datasets with up to 4B images and 30k classes our method requires 14X fewer additional parameters, does not require tuning the temperature on a held-out set and performs consistently better than the baseline heteroscedastic classifier. HET-XL improves ImageNet 0-shot classification in a multimodal contrastive learning setup which can be viewed as a 3.5 billion class classification problem.

==> diagram.tex <==
\subfigure[Vanilla \texttt{HET}]{

\scalebox{0.7}{

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,144); %set diagram left start at 0, and has height of 144

%Rounded Rect [id:dp8048264847979779] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (202.3,51.8) .. controls (202.3,48.71) and (204.81,46.2) .. (207.9,46.2) -- (267.7,46.2) .. controls (270.79,46.2) and (273.3,48.71) .. (273.3,51.8) -- (273.3,68.6) .. controls (273.3,71.69) and (270.79,74.2) .. (267.7,74.2) -- (207.9,74.2) .. controls (204.81,74.2) and (202.3,71.69) .. (202.3,68.6) -- cycle ;

%Rounded Rect [id:dp3741878447476211] 
\draw[rounded corners,fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1] (98, 10) rectangle (140, 110) {};

%Shape: Circle [id:dp9992654626407754] 
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(120, 30) circle (8pt);
%Shape: Circle [id:dp7735833740146072] 
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(120, 90) circle (8pt);
%Shape: Circle [id:dp27952725131624245] 
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(120, 60) circle (8pt);

%Image [id:dp6430614988355561] 
%\draw (45.72,58.4) node  {\includegraphics[width=56.89pt,height=39.9pt]{iclr2023/images/dog.jpeg}};
\draw (25.72,58.4) node  {\includegraphics[width=56.89pt,height=39.9pt]{iclr2023/images/dog.jpeg}};

%Rounded Rect [id:dp7736397466642132] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (332.8,51.6) .. controls (332.8,48.07) and (335.67,45.2) .. (339.2,45.2) -- (443.4,45.2) .. controls (446.93,45.2) and (449.8,48.07) .. (449.8,51.6) -- (449.8,70.8) .. controls (449.8,74.33) and (446.93,77.2) .. (443.4,77.2) -- (339.2,77.2) .. controls (335.67,77.2) and (332.8,74.33) .. (332.8,70.8) -- cycle ;

%Straight Lines [id:da7624697547953498] 
\draw    (60.3,59.7) -- (89.3,59.7) ;
\draw [shift={(95.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da432758314701002] 
\draw    (141.3,59.7) -- (200.3,59.7) ;
\draw [shift={(202.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6561451037183686] 
\draw    (273.3,59.7) -- (328.8,59.7) ;
\draw [shift={(330.8,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0993478389421999] 
\draw    (451.3,59.7) -- (478.3,59.7) ;
\draw [shift={(480.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (487,49.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
u\ =\ W^{\top } \ \phi ( x) \ +\ \epsilon ( x) ,\ W\ \in \ \mathbb{R}^{D\ \times \ K} \ \\
\epsilon \ \sim \ \mathcal{N}( 0,\ \Sigma ( x)) ,\ \Sigma ( x) \ \in \ \mathbb{R}^{K\ \times \ \ K} \ 
\end{array}$};
% Text Node
\draw (152.3,18.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ $};
% Text Node
\draw (271.3,15.46) node [anchor=north west][inner sep=0.75pt]    {$W^{\top } \ \phi ( x) \ $};
% Text Node
\draw (219.72,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {logits};
% Text Node
\draw (352,53.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {noise injection};
% Text Node
\draw (-15,94.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {input image};
% Text Node
\draw (96,122.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {network};


\end{tikzpicture}


}
}
\subfigure[\texttt{HET-XL}]{
\scalebox{0.7}{

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,151); %set diagram left start at 0, and has height of 151

%Rounded Rect [id:dp8048264847979779]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (382.3,51.8) .. controls (382.3,48.71) and (384.81,46.2) .. (387.9,46.2) -- (447.7,46.2) .. controls (450.79,46.2) and (453.3,48.71) .. (453.3,51.8) -- (453.3,68.6) .. controls (453.3,71.69) and (450.79,74.2) .. (447.7,74.2) -- (387.9,74.2) .. controls (384.81,74.2) and (382.3,71.69) .. (382.3,68.6) -- cycle ;

%Rounded Rect [id:dp3741878447476211]
\draw[rounded corners,fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1] (118, 10) rectangle (160, 110) {};
%Shape: Circle [id:dp9992654626407754]
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(140, 30) circle (8pt);
%Shape: Circle [id:dp7735833740146072]
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(140, 60) circle (8pt);
%Shape: Circle [id:dp27952725131624245]
\draw [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] 
(140, 90) circle (8pt);

%Image [id:dp6430614988355561]
\draw (45.72,58.4) node  {\includegraphics[width=56.89pt,height=39.9pt]{iclr2023/images/dog.jpeg}};

%Rounded Rect [id:dp7736397466642132]
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (205.8,50.6) .. controls (205.8,47.07) and (208.67,44.2) .. (212.2,44.2) -- (316.4,44.2) .. controls (319.93,44.2) and (322.8,47.07) .. (322.8,50.6) -- (322.8,69.8) .. controls (322.8,73.33) and (319.93,76.2) .. (316.4,76.2) -- (212.2,76.2) .. controls (208.67,76.2) and (205.8,73.33) .. (205.8,69.8) -- cycle ;

%Straight Lines [id:da7624697547953498]
\draw    (84.3,59.7) -- (111.3,59.7) ;
\draw [shift={(113.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da432758314701002]
\draw    (163.3,59.7) -- (200.3,59.7) ;
\draw [shift={(202.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6561451037183686]
\draw    (324.3,59.7) -- (379.8,59.7) ;
\draw [shift={(381.8,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0993478389421999]
\draw    (455.3,59.7) -- (482.3,59.7) ;
\draw [shift={(484.3,59.7)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (487,49.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
u\ =\ W^{\top } \ ( \phi ( x) \ +\ \epsilon^\prime ( x)) ,\ W\ \in \ \mathbb{R}^{D\ \times \ K} \ \\
\epsilon \ \sim \ \mathcal{N}( 0,\ \Sigma^\prime ( x)) ,\ \Sigma^\prime ( x) \ \in \ \mathbb{R}^{D\times D} \
\end{array}$};
% Text Node
\draw (172.3,18.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ $};
% Text Node
\draw (313.3,16.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ +\epsilon ( x) \ $};
% Text Node
\draw (399.72,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {logits};
% Text Node
\draw (225,52.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {noise injection};
% Text Node
\draw (5,94.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {input image};
% Text Node
\draw (116,122.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {network};


\end{tikzpicture}


}
}

==> diagram_backup.tex <==
\subfigure[Vanilla \texttt{HET}]{

\scalebox{0.7}{

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,388); %set diagram left start at 0, and has height of 388

%Rounded Rect [id:dp8048264847979779] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (69.3,172.8) .. controls (69.3,169.71) and (71.81,167.2) .. (74.9,167.2) -- (181.7,167.2) .. controls (184.79,167.2) and (187.3,169.71) .. (187.3,172.8) -- (187.3,189.6) .. controls (187.3,192.69) and (184.79,195.2) .. (181.7,195.2) -- (74.9,195.2) .. controls (71.81,195.2) and (69.3,192.69) .. (69.3,189.6) -- cycle ;

%Rounded Rect [id:dp3741878447476211] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (177.14,235.85) .. controls (182.03,235.85) and (186,239.82) .. (186,244.71) -- (186,271.29) .. controls (186,276.18) and (182.03,280.15) .. (177.14,280.15) -- (92.86,280.15) .. controls (87.97,280.15) and (84,276.18) .. (84,271.29) -- (84,244.71) .. controls (84,239.82) and (87.97,235.85) .. (92.86,235.85) -- cycle ;
%Shape: Circle [id:dp9992654626407754] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (166,246.6) .. controls (172.3,246.6) and (177.4,251.7) .. (177.4,258) .. controls (177.4,264.3) and (172.3,269.4) .. (166,269.4) .. controls (159.7,269.4) and (154.6,264.3) .. (154.6,258) .. controls (154.6,251.7) and (159.7,246.6) .. (166,246.6) -- cycle ;
%Shape: Circle [id:dp7735833740146072] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (104,247.6) .. controls (110.3,247.6) and (115.4,252.7) .. (115.4,259) .. controls (115.4,265.3) and (110.3,270.4) .. (104,270.4) .. controls (97.7,270.4) and (92.6,265.3) .. (92.6,259) .. controls (92.6,252.7) and (97.7,247.6) .. (104,247.6) -- cycle ;
%Shape: Circle [id:dp27952725131624245] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (136,246.6) .. controls (142.3,246.6) and (147.4,251.7) .. (147.4,258) .. controls (147.4,264.3) and (142.3,269.4) .. (136,269.4) .. controls (129.7,269.4) and (124.6,264.3) .. (124.6,258) .. controls (124.6,251.7) and (129.7,246.6) .. (136,246.6) -- cycle ;

%Straight Lines [id:da9893227423161812] 
\draw    (131,318) -- (131,288) ;
\draw [shift={(131,286)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Image [id:dp48129108557771216] 
\draw (132.72,346.4) node  {\includegraphics[width=56.89pt,height=39.9pt]{iclr2023/images/dog.jpeg}};

%Rounded Rect [id:dp7736397466642132] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (69.8,101.6) .. controls (69.8,98.07) and (72.67,95.2) .. (76.2,95.2) -- (180.4,95.2) .. controls (183.93,95.2) and (186.8,98.07) .. (186.8,101.6) -- (186.8,120.8) .. controls (186.8,124.33) and (183.93,127.2) .. (180.4,127.2) -- (76.2,127.2) .. controls (72.67,127.2) and (69.8,124.33) .. (69.8,120.8) -- cycle ;

%Straight Lines [id:da5017301584880602] 
\draw    (131.5,233.2) -- (131.31,204.2) ;
\draw [shift={(131.3,202.2)}, rotate = 89.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4028973243750703] 
\draw    (132,164.2) -- (132,134.2) ;
\draw [shift={(132,132.2)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7624697547953498] 
\draw    (131,93.2) -- (131.28,56.2) ;
\draw [shift={(131.3,54.2)}, rotate = 90.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp66561496395919] 
\draw  [dash pattern={on 1.69pt off 2.76pt}][line width=1.5]  (29.8,69.2) -- (230.8,69.2) -- (230.8,202.2) -- (29.8,202.2) -- cycle ;

% Text Node
\draw (22,7.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
u\ =\ W^\top\ \phi ( x) \ +\ \epsilon ( x) ,\ W\ \in \ \mathbb{R}^{D \times  K} \ \\
\epsilon(x) \ \sim \ \mathcal{N}( 0,\ \Sigma ( x)) ,\ \Sigma ( x) \ \in \ \mathbb{R}^{K \times K} \ 
\end{array}$};
% Text Node
\draw (88.3,208.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ $};
% Text Node
\draw (65.3,138.46) node [anchor=north west][inner sep=0.75pt]    {$W^\top\ \phi ( x) \ $};
% Text Node
\draw (107,80.4) node [anchor=north west][inner sep=0.75pt]    {$u$};
% Text Node
\draw (110.5,174) node [anchor=north west][inner sep=0.75pt]   [align=left] {logits};
% Text Node
\draw (90,103.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {noise injection};
% Text Node
\draw (170,210) node [anchor=north west][inner sep=0.75pt]   [align=left] {MC sampling};
% Text Node
\draw (5,338.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {input image};
% Text Node
\draw (19,249.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {network};


\end{tikzpicture}

}
}
\hfill
\subfigure[\texttt{HET-XL}]{
\scalebox{0.7}{

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,404); %set diagram left start at 0, and has height of 404

%Straight Lines [id:da1879923191899877] 
\draw    (127.85,244.2) -- (127.66,215.2) ;
\draw [shift={(127.65,213.2)}, rotate = 89.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8422865537529558] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (69.3,114.8) .. controls (69.3,111.71) and (71.81,109.2) .. (74.9,109.2) -- (181.7,109.2) .. controls (184.79,109.2) and (187.3,111.71) .. (187.3,114.8) -- (187.3,131.6) .. controls (187.3,134.69) and (184.79,137.2) .. (181.7,137.2) -- (74.9,137.2) .. controls (71.81,137.2) and (69.3,134.69) .. (69.3,131.6) -- cycle ;

%Rounded Rect [id:dp2723793923955036] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (70.8,182.6) .. controls (70.8,179.07) and (73.67,176.2) .. (77.2,176.2) -- (181.4,176.2) .. controls (184.93,176.2) and (187.8,179.07) .. (187.8,182.6) -- (187.8,201.8) .. controls (187.8,205.33) and (184.93,208.2) .. (181.4,208.2) -- (77.2,208.2) .. controls (73.67,208.2) and (70.8,205.33) .. (70.8,201.8) -- cycle ;
%Straight Lines [id:da8177367741506433] 
\draw    (127.75,175.2) -- (127.75,145.2) ;
\draw [shift={(127.75,143.2)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp07447705599436583] 
\draw  [dash pattern={on 1.69pt off 2.76pt}][line width=1.5]  (26.8,82.2) -- (227.8,82.2) -- (227.8,215.2) -- (26.8,215.2) -- cycle ;
%Straight Lines [id:da8119926004586683] 
\draw    (127.6,107.2) -- (127.88,70.2) ;
\draw [shift={(127.9,68.2)}, rotate = 90.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp10098801027238169] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (175.14,246.85) .. controls (180.03,246.85) and (184,250.82) .. (184,255.71) -- (184,282.29) .. controls (184,287.18) and (180.03,291.15) .. (175.14,291.15) -- (90.86,291.15) .. controls (85.97,291.15) and (82,287.18) .. (82,282.29) -- (82,255.71) .. controls (82,250.82) and (85.97,246.85) .. (90.86,246.85) -- cycle ;
%Shape: Circle [id:dp13485650277354144] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (164,257.6) .. controls (170.3,257.6) and (175.4,262.7) .. (175.4,269) .. controls (175.4,275.3) and (170.3,280.4) .. (164,280.4) .. controls (157.7,280.4) and (152.6,275.3) .. (152.6,269) .. controls (152.6,262.7) and (157.7,257.6) .. (164,257.6) -- cycle ;
%Shape: Circle [id:dp9569752409780191] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (102,258.6) .. controls (108.3,258.6) and (113.4,263.7) .. (113.4,270) .. controls (113.4,276.3) and (108.3,281.4) .. (102,281.4) .. controls (95.7,281.4) and (90.6,276.3) .. (90.6,270) .. controls (90.6,263.7) and (95.7,258.6) .. (102,258.6) -- cycle ;
%Shape: Circle [id:dp5463705530058229] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (134,257.6) .. controls (140.3,257.6) and (145.4,262.7) .. (145.4,269) .. controls (145.4,275.3) and (140.3,280.4) .. (134,280.4) .. controls (127.7,280.4) and (122.6,275.3) .. (122.6,269) .. controls (122.6,262.7) and (127.7,257.6) .. (134,257.6) -- cycle ;

%Straight Lines [id:da6847252418958795] 
\draw    (129,329) -- (129,299) ;
\draw [shift={(129,297)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Image [id:dp7689767374188251] 
\draw (130.72,357.4) node  {\includegraphics[width=56.89pt,height=39.9pt]{iclr2023/images/dog.jpeg}};


% Text Node
\draw (15,16) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
u\ =\ W^\top\ ( \phi ( x) \ +\ \epsilon^\prime ( x)) ,\ W\ \in \ \mathbb{R}^{D \times K} \ \\
\epsilon^\prime(x) \ \sim \ \mathcal{N}( 0,\ \Sigma^\prime ( x)) ,
%\Sigma ( x) \ =\ W^\top \Sigma^\prime ( x) W ,
\ \Sigma^\prime ( x) \in \ \mathbb{R}^{D \times D} \ 
\end{array}$};
% Text Node
\draw (88.3,219.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ $};
% Text Node
\draw (90,184.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {noise injection};
% Text Node
\draw (33.3,149.46) node [anchor=north west][inner sep=0.75pt]    {$\phi ( x) \ +\ \epsilon ( x) \ $};
% Text Node
\draw (104,94.4) node [anchor=north west][inner sep=0.75pt]    {$u$};
% Text Node
\draw (110.5,116) node [anchor=north west][inner sep=0.75pt]   [align=left] {logits};
% Text Node
\draw (177,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {MC sampling};
% Text Node
\draw (17,260.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {network};
% Text Node
\draw (3,349.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {input image};


\end{tikzpicture}


}
}

==> tuning_tau_backup.tex <==
As described in \Cref{sec:background_mcsamples_temp}, the temperature parameter $\tau$ in the approach of \citet{collier2020simple} controls a bias-variance trade-off. The resulting performance is sensitive to the temperature value, whose selection generally varies from one dataset to another \citep{collier2020simple,collier2021correlated}. In practice, this additional hyperparameter is included in the hyperparameter sweep. However, especially at scales considered in this paper, it can be tedious, if not impossible, to run such a sweep. At the same time, bypassing this step or making the sweep too coarse may degrade the performance \citep{collier2020simple}.
We therefore investigate strategies to automatically and efficiently tune the temperature $\tau$.

\subsection{The specific structure of the hyperparameter $\tau$}\label{sec:structure_hyperparameter_tau}

The temperature $\tau$ has the property to explicitly appear both at training and validation time, unlike optimisation-related or regularisation-related hyperparameters that surface only at training time. As we next see, this observation has implications about the way we can compute a gradient estimator to tune $\tau$.

To ease the exposition, let us momentarily simplify our setup. We consider a temperature-scaled model $1/\tau \cdot f(\vx; \Theta) \in \R$ with a one-dimensional output, e.g., in a regression task. The parameters of the model are summarised in $\Theta \in \R^P$. Moreover, let $\gL_\text{train}(\cdot, \cdot)$ and $\gL_\text{val}(\cdot, \cdot)$ be two loss functions, defined respectively for training data $(\vx, y) \sim p_\text{train}$ and validation data $(\vx, y) \sim p_\text{val}$.
%
We typically seek a temperature parameter that minimises some validation objective in a bi-level optimisation formulation~\citep{franceschi2018bilevel}
\begin{equation}\label{eq:bilevel_validation_loss}
    \min_{\tau > 0} \
    F_\text{val}(\tau)
    \quad\text{with}\quad
    F_\text{val}(\tau) = 
    \E_{(\vx, y) \sim p_\text{val}}\left[ \gL_\text{val}\left(\frac{1}{\tau} \cdot f(\vx; \Theta^*(\tau)), y\right)\right] 
\end{equation}
for some parameters $\Theta^*(\tau)$ defined as a solution of the training problem
\begin{equation}\label{eq:bilevel_training_loss}
    \Theta^*(\tau) \in \argmin_{\Theta \in \R^P} \ F_\text{train}(\tau, \Theta)
    \quad\text{with}\quad
    F_\text{train}(\tau, \Theta) = 
    \E_{(\vx, y) \sim p_\text{train}}\left[ \gL_\text{train}\left(\frac{1}{\tau} \cdot f(\vx; \Theta), y \right)\right].
\end{equation}
It can be shown (see \Cref{sec:appendix_tuning_tau}) that by applying the chain rule, we can compute the gradient of the objective in \cref{eq:bilevel_validation_loss} for a given pair $(\vx, y)$ of the expectation, leading to:
\begin{equation}\label{eq:bilevel_gradient}
\frac{\partial \gL_\text{val}(y', y)}{\partial y'} \Big|_{y'= \frac{1}{\tau} f(\vx; \Theta^*(\tau))}
\cdot
\left\{
  {\color{orange}-\frac{1}{\tau^2} f(\vx; \Theta^*(\tau))} + \frac{1}{\tau} 
  \big\langle \nabla_\Theta f(\vx; \Theta) \big|_{\Theta = \Theta^*(\tau)}, 
  {\color{red} \nabla_\tau \Theta^*(\tau) }\big\rangle
\right\}.
\end{equation}
In the expression above, the most complex term to handle is 
{\color{red} $\nabla_\tau \Theta^*(\tau)$} since it requires to differentiate through the solution of another optmization problem, notably involving higher-order derivatives~\citep{maclaurin2015gradient,luketina2016scalable,pedregosa2016hyperparameter,franceschi2018bilevel,lorraine2020optimizing}. 

Several approaches have been proposed to approximate this term. For example, \citet{luketina2016scalable} only consider the hyperparameter influence through the current gradient step solving \cref{eq:bilevel_training_loss}. This formally translates into  ${\color{red}\nabla_\tau \Theta^*(\tau)} \approx -s_t \cdot \nabla_{\tau}[\nabla_{\Theta} F_\text{train}(\tau, \Theta_t)]$ with $s_t$ and $\Theta_t$ being respectively the learning rate and iterate produced at step $t$ by an iterative algorithm solving \cref{eq:bilevel_training_loss}, e.g., SGD. In our comparison, we will take \citet{luketina2016scalable} as a representative approach for efficient gradient-based hyperparameter tuning.

\textbf{A simple gradient estimator.}
A remarkable property of the temperature is that $F_\text{val}$ in \cref{eq:bilevel_validation_loss} depends on $\tau$ not only through $\Theta^*(\tau)$---as it would be for example the case for weight decay---but also directly via $1/\tau$.
%
While in absence of this property, the gradient of $F_\text{val}$ would solely rely on ${\color{red}\nabla_\tau \Theta^*(\tau)}$, 
in the case of $\tau$, we can assume that ${\color{red}\nabla_\tau \Theta^*(\tau)}=0$ (i.e., the optimal $\Theta^*(\tau)$ mildly varies with $\tau$) and focus on {\color{orange} $-\frac{1}{\tau^2} f(\vx; \Theta^*(\tau))$} for the gradient.
%
Interestingly, further approximating $\Theta^*(\tau) \approx \Theta_t$, the resulting estimator is extremely simple and cheap to compute, e.g., no higher-order derivatives to compute. Moreover, we can notice that, provided that $\gL_\text{train}=\gL_\text{val}$ (in our comparison, both are set to the negative log likelihood) and the training and validation sets are identical, $-\frac{1}{\tau^2} f(\vx; \Theta_t)$ falls back to the gradient we would take by treating $\tau$ as a standard training parameter by directly solving $\min_{\tau>0, \Theta \in \R^P} F_\text{train}(\tau, \Theta)$.  



% Interestingly, since the validation objective \cref{eq:bilevel_validation_loss} depends on $\tau$ not only through $\Theta^*(\tau)$---as it would be for example the case for weight decay---we can approximate the gradient \cref{eq:bilevel_gradient} of \cref{eq:bilevel_validation_loss} by discarding the most complex term {\color{red} $\nabla_\tau \Theta^*(\tau)$} whose differentiation raises multiple challenges~\citep{maclaurin2015gradient,luketina2016scalable,pedregosa2016hyperparameter,franceschi2018bilevel,lorraine2020optimizing}. 
% We will thus consider a simple approach solely based on {\color{orange} $-\frac{1}{\tau^2} f(\vx; \Theta^*(\tau))$} (i.e.,  ${\color{red}\nabla_\tau \Theta^*(\tau)}=0$) where we approximate $\Theta^*(\tau)$ by $\Theta_t(\tau)$, the iterate produced at step $t$ by the iterative algorithm, e.g., SGD, while solving \cref{eq:bilevel_training_loss}. Despite the naivety of the approximation, as we will see, this approach is competitive.

% \citet{luketina2016scalable} approximate $\Theta^*(\tau)$ by considering the dependency of $\tau$ only in the last iterate $\Theta_t(\tau)$ obtained by the iterative algorithm, e.g., SGD, solving \cref{eq:bilevel_training_loss}.

\subsection{Do we need a validation set?}\label{sec:do_we_need_a_validation_set}

The experiments we consider in \Cref{sec:results} bring into play datasets with a large number of data points (from 12.8M up to 4B) over which the training performs only a few epochs.
As a result, it is natural to wonder to what extent metrics collected on the training set are faithful to metrics computed on a proper held-out validation set.
%
In the perspective of providing a simple approach to tune $\tau$ that would not hinder the deployment of \texttt{HET-XL}, e.g., without having to define a held-out validation set, we explore the impact of directly tuning $\tau$ on the training set.

\subsection{A case study}

The two previous sections indicate that the particular structure of $\tau$ (\Cref{sec:structure_hyperparameter_tau}) and the large-scale training regime (\Cref{sec:do_we_need_a_validation_set}) can lead to simple approaches to tune $\tau$. 
We study if there is any opportunity cost in applying those simple approaches when compared with more sophisticated methods of the literature.   

\RJ{TODO: Add details about the setting (ResNet50x2 on ImageNet-21k for 7 epochs, a scaled-down setting faithful to the experiments of \Cref{sec:results}, 3 folds)}

\RJ{TODO: Add discussion; there is no opportunity cost in using the simplest approach (tuning $\tau$ as a standard training parameter), even when compared to more complex (e.g., \citet{luketina2016scalable}) and more expensive techniques like Bayesian optimization (BO) requiring multiple trainings.}

\RJ{TODO: Secondary observations. (i) Not useful to retrain, (ii) there is some overfitting happening while tuning for NLL, (iii) having a better gradient estimate seems to make a difference}

\RJ{TODO: Add details in the appendix about the other baselines.}

\begin{table}[]
    \centering
    \caption{Comparison of different approaches to tune $\tau$ for a ResNet50x2 on ImageNet-21k.}
    \scalebox{0.92}{
\begin{tabular}{lcccc}
\toprule
                                \textbf{Method} &              \textbf{$\downarrow$NLL} &               \textbf{$\uparrow$Prec@1} &  \textbf{Single training?} & \textbf{No val.~set needed?} \\
\midrule
                                    Grid search &  6.08 {\tiny \color{gray} $\pm$ 0.04} &  0.433 {\tiny \color{gray} $\pm$ 0.002} &      {\color{red}$\times$} &        {\color{red}$\times$} \\
                          Bayesian optimization &  6.03 {\tiny \color{gray} $\pm$ 0.06} &  0.428 {\tiny \color{gray} $\pm$ 0.000} &      {\color{red}$\times$} &        {\color{red}$\times$} \\
                          \midrule
                         Luketina et al.~(2016) &  6.08 {\tiny \color{gray} $\pm$ 0.04} &  0.425 {\tiny \color{gray} $\pm$ 0.000} &  {\color{green}\checkmark} &        {\color{red}$\times$} \\
                          Simple gradient (val) &  6.22 {\tiny \color{gray} $\pm$ 0.05} &  0.432 {\tiny \color{gray} $\pm$ 0.001} &  {\color{green}\checkmark} &        {\color{red}$\times$} \\

 Simple gradient (train, as in \texttt{HET-XL}) &  5.99 {\tiny \color{gray} $\pm$ 0.04} &  0.435 {\tiny \color{gray} $\pm$ 0.001} &  {\color{green}\checkmark} &    {\color{green}\checkmark} \\
\bottomrule
\end{tabular}
}
    \label{tab:my_label}
\end{table}



% TODO(rjenatton): Move the full derivations in the appendix.
% \begin{align*}
% \nabla_\tau \left[
% \gV\left(\frac{1}{\tau} f(\vx; \Theta^*(\tau)), y\right)
% \right]
% &= \frac{\partial \gV(y', y)}{\partial y'} \Big|_{y'= \frac{1}{\tau} f(\vx; \Theta^*(\tau))}
% \cdot \nabla_\tau \left[\frac{1}{\tau} f(\vx; \Theta^*(\tau)), y)\right] \\
% &=
% \frac{\partial \gV(y', y)}{\partial y'} \Big|_{y'= \frac{1}{\tau} f(\vx; \Theta^*(\tau))}
% \cdot
% \left\{
%   -\frac{1}{\tau^2} f(\vx; \Theta^*(\tau)) + \frac{1}{\tau} 
%   \langle \nabla_\Theta f(\vx; \Theta) \big|_{\Theta = \Theta^*(\tau)}, 
%   {\color{red} \nabla_\tau \Theta^*(\tau) }\rangle
% \right\}
% \end{align*} 

% \MC{Should we add a short description of why this specific structure makes the learning of $\tau$ more reasonable than other hyperparameters and connect this to (i) the dataset scale e.g.\ @rjenatton's argument that 1 epoch ~= tune on val set and (ii) the existing hyperparameter learning literature?}

% [BEGIN] Mark's previous section
% \section{Learning $\tau$}

% The temperature parameter $\tau$ of the HET and HET-X methods, controls a bias/variance tradeoff in the approximation to the assumed generative process \citep{collier2020simple}. The resulting performance is typically sensitive to the temperature value, whose selection generally varies from one dataset to another \citep{collier2020simple,collier2021correlated}. In practice the additional hyperparameter is included in the hyperparameter sweep. However, especially at scales considered in this paper, it can be tedious and expensive to run such a sweep. Bypassing this step or making the sweep too coarse may degrade the performance \citep{collier2020simple}.

% [Rodolphe I am not 100\% sure how best to present the mathematical argument for the temperature learning, I have only added the intro.]
% [END] Mark's previous section
